Routing on Sparse Graphs with Non-metric Costs for the Prize-collecting Travelling Salesperson Problem

In many real-world routing problems, decision makers must optimise over sparse graphs such as transportation networks with non-metric costs on the edges that do not obey the triangle inequality. Motivated by finding a sufficiently long running route in a city that minimises the air pollution exposure of the runner, we study the Prize-collecting Travelling Salesperson Problem (Pc-TSP) on sparse graphs with non-metric costs. Given an undirected graph with a cost function on the edges and a prize function on the vertices, the goal of Pc-TSP is to find a tour rooted at the origin that minimises the total cost such that the total prize is at least some quota. First, we introduce heuristics designed for sparse graphs with non-metric cost functions where previous work dealt with either a complete graph or a metric cost function. Next, we develop a branch & cut algorithm that employs a new cut we call the disjoint-paths cost-cover (DPCC) cut. Empirical experiments on two datasets show that our heuristics can produce a feasible solution with less cost than a state-of-the-art heuristic from the literature. On datasets with non-metric cost functions, DPCC is found to solve more instances to optimality than the baseline cutting algorithm we compare against.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> tables/LAQ_compare_heuristics_extra.tex <==
\begin{tabular}{l
    S[table-format=1.2e3]S[round-mode=places,round-precision=3,scientific-notation=false,table-format=1.3]rc    
    S[table-format=1.2e3]S[round-mode=places,round-precision=3,scientific-notation=false,table-format=1.3]rc
    S[table-format=1.2e3]S[round-mode=places,round-precision=3,scientific-notation=false,table-format=1.3]rc
    S[table-format=1.2e3]S[round-mode=places,round-precision=3,scientific-notation=false,table-format=1.3]r}
\toprule
{} & \multicolumn{3}{c}{BFS-EC} && \multicolumn{3}{c}{BFS-PEC} && \multicolumn{3}{c}{SBL} && \multicolumn{3}{c}{SBL-PEC}\\\cmidrule{2-4}\cmidrule{6-8}\cmidrule{10-12}\cmidrule{14-16}
{Quota} & {$\overline{\text{TIME}}$ (s)} & {$\overline{\text{GAP}}$} & {FEAS} && {$\overline{\text{TIME}}$ (s)} & {$\overline{\text{GAP}}$} & {FEAS} && {$\overline{\text{TIME}}$ (s)} & {$\overline{\text{GAP}}$} & {FEAS} && {$\overline{\text{TIME}}$ (s)} & {$\overline{\text{GAP}}$} & {FEAS} \\
\midrule
1000 & 6.196139 & 0.066245{$^\star$} & 3 && 25.004115 & 4.909803{$^\star$} & 4 && 6.216024 & 0.000000{$^\star$} & 4 && 24.871107 & 0.000000{$^\star$} & 4 \\
2000 & 6.296389 & 0.000000{$^\star$} & 1 && 21.010743 & 9.585612{$^\star$} & 4 && 6.306077 & 0.039909{$^\star$} & 4 && 30.170955 & 0.039909{$^\star$} & 4 \\
3000 & 6.364708 & nan & 0 && 47.275385 & 19.618502{$^\star$} & 4 && 6.242654 & 0.027181{$^\star$} & 4 && 31.523599 & 0.027181{$^\star$} & 4 \\
4000 & 6.134155 & nan & 0 && 59.535590 & 16.263189{$^\star$} & 4 && 6.111517 & 0.048623{$^\star$} & 4 && 29.297383 & 0.048623{$^\star$} & 4 \\
5000 & 6.076099 & nan & 0 && 54.874739 & 13.842067 & 4 && 6.103824 & 0.116738 & 4 && 30.025093 & 0.116738 & 4 \\
\bottomrule
\end{tabular}


==> tables/tspwplib_compare_heuristics_SBL-EC.tex <==
\begin{tabular}{ll
    S[scientific-notation=false,round-mode=places,round-precision=1]
    S[round-mode=places,round-precision=3,scientific-notation=false,table-format=1.3]
    r
}
\toprule
{} & {} & \multicolumn{3}{c}{SBL-EC} \\\cmidrule{3-5}
{Cost} & {$\kappa$} & {$\overline{\text{TIME}}$ (s)} & {$\overline{\text{GAP}}$} & {FEAS} \\
\midrule
EUC & 5 & 0.199719 & 1.398531 & 42 \\
 & 10 & 1.744754 & 2.535878 & 93 \\
 & 15 & 16.008364 & 3.372375 & 121 \\
 & 20 & 29.382611 & 3.593715 & 120 \\
 & 25 & 37.782733 & 2.918703 & 121 \\
MST & 5 & 0.256310 & 3.325319 & 62 \\
 & 10 & 2.327281 & 6.108636 & 97 \\
 & 15 & 15.318947 & 6.617239 & 125 \\
 & 20 & 27.933670 & 6.141395 & 133 \\
 & 25 & 36.665531 & 5.622649 & 133 \\
\bottomrule
\end{tabular}


==> tables/tspwplib_disjoint_paths.tex <==
\begin{tabular}{lrr}
    \toprule
    {$\alpha$} & {EUC} & {MST} \\
    \midrule
    0.05 & 16 & 0 \\
    0.10 & 54 & 24 \\
    0.25 & 118 & 105 \\
    0.50 & 135 & 133 \\
    0.75 & 135 & 135 \\
\end{tabular}
